Impact of Extensions on Browser Performance: An Empirical Study on Google Chrome

Web browsers have been used widely by users to conduct various online activities, such as information seeking or online shopping. To improve user experience and extend the functionality of browsers, practitioners provide mechanisms to allow users to install third-party-provided plugins (i.e., extensions) on their browsers. However, little is known about the performance implications caused by such extensions. In this paper, we conduct an empirical study to understand the impact of extensions on the user-perceived performance (i.e., energy consumption and page load time) of Google Chrome, the most popular browser. We study a total of 72 representative extensions from 11 categories (e.g., Developer Tools and Sports). We observe that browser performance can be negatively impacted by the use of extensions, even when the extensions are used in unintended circumstances (e.g., when logging into an extension is not granted but required, or when an extension is not used for designated websites). We also identify a set of factors that significantly influence the performance impact of extensions, such as code complexity and privacy practices (i.e., collection of user data) adopted by the extensions. Based on our empirical observations, we provide recommendations for developers and users to mitigate the performance impact of browser extensions, such as conducting performance testing and optimization for unintended usage scenarios of extensions, or adhering to proper usage practices of extensions (e.g., logging into an extension when required).

==> tables/clusters2.tex <==
% \usepackage{graphicx}
% \usepackage{multirow}
% \usepackage{booktabs}


% \begin{table}
% \centering
% \caption{\bihui{R1.18 - Obtained clusters}.}
% \vspace{-2mm}
% \label{tab:clusters}
% % \SetTblrInner{rowsep=0pt}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{clcl} 
% \toprule
% Cluster & \multicolumn{1}{c}{Privacy Practice} & Number & Total \\ 
% \hline
% 0 & None & 31908 & 31908 \\ \hline
% \multirow{22}{*}{1} & Website content & 3412 & \multirow{22}{*}{4056} \\
%  & Website content, Authentication information & 213 &  \\
%  & Website content, Web history & 206 &  \\
%  & Location, Website content & 88 &  \\
%  & Website content, Personal communications & 42 &  \\
%  & Location, Website content, Web history & 36 &  \\
%  & Location, Website content, Authentication information & 10 &  \\
%  & Website content, Authentication information, Personal communications & 10 &  \\
%  & Website content, Web history, Authentication information & 10 &  \\
%  & Website content, Web history, Personal communications & 6 &  \\
%  & Location, Website content, Web history, Authentication information & 4 &  \\
%  & Website content, Financial and payment information & 4 &  \\
%  & Location, Website content, Financial and payment information & 2 &  \\
%  & Location, Website content, Personal communications & 2 &  \\
%  & Website content, Authentication information, Financial and payment information & 2 &  \\
%  & Website content, Web history, Authentication information, Personal communications & 2 &  \\
%  & Website content, Web history, Financial and payment information & 2 &  \\
%  & Location, Website content, Authentication information, Personal communications & 1 &  \\
%  & Location, Website content, Web history, Personal communications & 1 &  \\
%  & Website content, Health information & 1 &  \\
%  & Website content, Web history, Authentication information, Health information & 1 &  \\
%  & Website content, Web history, Personal communications, Health information & 1 &  \\ 
% \hline
% \multirow{61}{*}{2} & Authentication information & 492 & \multirow{61}{*}{1951} \\
%  & P.I.I., Authentication information & 432 &  \\
%  & Website content, P.I.I., Authentication information & 301 &  \\
%  & User activity, P.I.I., Authentication information & 79 &  \\
%  & P.I.I., Authentication information, Personal communications & 57 &  \\
%  & Location, P.I.I., Authentication information & 54 &  \\
%  & P.I.I., Authentication information, Financial and payment information & 54 &  \\
%  & Authentication information, Personal communications & 32 &  \\
%  & Web history, P.I.I., Authentication information & 31 &  \\
%  & Website content, P.I.I., Authentication information, Personal communications & 31 &  \\
%  & Location, Authentication information & 26 &  \\
%  & Location, Website content, P.I.I., Authentication information & 25 &  \\
%  & Location, P.I.I., Authentication information, Financial and payment information & 23 &  \\
%  & Location, User activity, P.I.I., Authentication information & 22 &  \\
%  & Website content, P.I.I., Authentication information, Financial and payment information & 22 &  \\
%  & Website content, Web history, P.I.I., Authentication information & 20 &  \\
%  & Location, P.I.I., Authentication information, Personal communications & 17 &  \\
%  & User activity, Web history, P.I.I., Authentication information & 17 &  \\
%  & Location, User activity, P.I.I., Authentication information, Financial and payment information & 16 &  \\
%  & P.I.I., Authentication information, Personal communications, Financial and payment information & 16 &  \\
%  & User activity, P.I.I., Authentication information, Financial and payment information & 16 &  \\
%  & Location, Website content, Web history, P.I.I., Authentication information & 15 &  \\
%  & Web history, Authentication information & 15 &  \\
%  & Authentication information, Financial and payment information & 13 &  \\
%  & User activity, P.I.I., Authentication information, Personal communications & 12 &  \\
%  & Website content, Web history, P.I.I., Authentication information, Personal communications & 10 &  \\
%  & Location, Website content, P.I.I., Authentication information, Personal communications & 7 &  \\
%  & Website content, P.I.I., Authentication information, Personal communications, Financial and payment information & 7 &  \\
%  & Location, User activity, P.I.I., Authentication information, Personal communications, Financial and payment information & 6 &  \\
%  & Location, User activity, Web history, P.I.I., Authentication information & 6 &  \\
%  & Location, Web history, P.I.I., Authentication information & 6 &  \\
%  & Location, P.I.I., Authentication information, Personal communications, Financial and payment information & 5 &  \\
%  & Web history, P.I.I., Authentication information, Financial and payment information & 5 &  \\
%  & Website content, Web history, P.I.I., Authentication information, Financial and payment information & 5 &  \\
%  & Authentication information, Personal communications, Financial and payment information & 4 &  \\
%  & Location, User activity, P.I.I., Authentication information, Personal communications & 4 &  \\
%  & Location, Web history, Authentication information & 4 &  \\
%  & Location, Web history, P.I.I., Authentication information, Financial and payment information & 4 &  \\
%  & Location, Website content, P.I.I., Authentication information, Financial and payment information & 4 &  \\
%  & Location, P.I.I., Authentication information, Financial and payment information, Health information & 3 &  \\
%  & Location, User activity, Web history, P.I.I., Authentication information, Personal communications, Financial and payment information & 3 &  \\
%  & Location, Web history, P.I.I., Authentication information, Personal communications & 3 &  \\
%  & Location, Authentication information, Personal communications & 2 &  \\
%  & Location, User activity, Web history, P.I.I., Authentication information, Financial and payment information & 2 &  \\
%  & Location, Website content, P.I.I., Authentication information, Personal communications, Financial and payment information & 2 &  \\
%  & P.I.I., Authentication information, Health information & 2 &  \\
%  & P.I.I., Authentication information, Personal communications, Health information & 2 &  \\
%  & Web history, Authentication information, Personal communications & 2 &  \\
%  & Web history, P.I.I., Authentication information, Personal communications & 2 &  \\
%  & Website content, Web history, P.I.I., Authentication information, Personal communications, Financial and payment information & 2 &  \\
%  & Location, Authentication information, Financial and payment information & 1 &  \\
%  & Location, P.I.I., Authentication information, Health information & 1 &  \\
%  & Location, P.I.I., Authentication information, Personal communications, Health information & 1 &  \\
%  & Location, User activity, Web history, P.I.I., Authentication information, Personal communications & 1 &  \\
%  & Location, Website content, Web history, P.I.I., Authentication information, Personal communications & 1 &  \\
%  & Location, Website content, Web history, P.I.I., Authentication information, Personal communications, Financial and payment information, Health information & 1 &  \\
%  & P.I.I., Authentication information, Personal communications, Financial and payment information, Health information & 1 &  \\
%  & User activity, P.I.I., Authentication information, Health information & 1 &  \\
%  & User activity, P.I.I., Authentication information, Personal communications, Financial and payment information & 1 &  \\
%  & User activity, Web history, P.I.I., Authentication information, Personal communications & 1 &  \\
%  & Website content, P.I.I., Authentication information, Health information & 1 &  \\ 
% \hline
% \multirow{59}{*}{3} & P.I.I. & 1490 & \multirow{59}{*}{3649} \\
%  & Website content, P.I.I. & 449 &  \\
%  & Web history & 368 &  \\
%  & Location & 338 &  \\
%  & User activity, P.I.I. & 121 &  \\
%  & Personal communications & 116 &  \\
%  & P.I.I., Personal communications & 107 &  \\
%  & Location, P.I.I. & 85 &  \\
%  & Web history, P.I.I. & 83 &  \\
%  & Location, Web history & 53 &  \\
%  & Website content, P.I.I., Personal communications & 52 &  \\
%  & Website content, Web history, P.I.I. & 46 &  \\
%  & Location, Website content, P.I.I. & 36 &  \\
%  & P.I.I., Financial and payment information & 34 &  \\
%  & Location, User activity, P.I.I. & 31 &  \\
%  & Location, Web history, P.I.I. & 23 &  \\
%  & Financial and payment information & 21 &  \\
%  & User activity, Web history, P.I.I. & 20 &  \\
%  & Location, Website content, Web history, P.I.I. & 15 &  \\
%  & Website content, P.I.I., Financial and payment information & 15 &  \\
%  & Location, Personal communications & 12 &  \\
%  & Location, P.I.I., Personal communications & 12 &  \\
%  & Location, User activity, Web history, P.I.I. & 12 &  \\
%  & Location, Website content, P.I.I., Personal communications & 12 &  \\
%  & User activity, P.I.I., Personal communications & 11 &  \\
%  & Health information & 8 &  \\
%  & Location, User activity, P.I.I., Personal communications & 8 &  \\
%  & User activity, P.I.I., Financial and payment information & 7 &  \\
%  & P.I.I., Personal communications, Financial and payment information & 6 &  \\
%  & Location, P.I.I., Financial and payment information & 5 &  \\
%  & P.I.I., Health information & 4 &  \\
%  & Website content, Web history, P.I.I., Personal communications & 4 &  \\
%  & Location, User activity, P.I.I., Personal communications, Financial and payment information & 3 &  \\
%  & Location, User activity, Web history, P.I.I., Personal communications & 3 &  \\
%  & Location, Web history, P.I.I., Personal communications & 3 &  \\
%  & Web history, Personal communications & 3 &  \\
%  & Location, P.I.I., Personal communications, Financial and payment information & 2 &  \\
%  & Location, User activity, Web history, P.I.I., Financial and payment information & 2 &  \\
%  & Location, Website content, P.I.I., Financial and payment information & 2 &  \\
%  & Location, Website content, P.I.I., Personal communications, Financial and payment information & 2 &  \\
%  & Location, Website content, Web history, P.I.I., Personal communications & 2 &  \\
%  & User activity, P.I.I., Personal communications, Financial and payment information & 2 &  \\
%  & Web history, P.I.I., Personal communications & 2 &  \\
%  & Website content, P.I.I., Health information & 2 &  \\
%  & Website content, P.I.I., Personal communications, Financial and payment information & 2 &  \\
%  & Website content, Web history, P.I.I., Financial and payment information & 2 &  \\
%  & Location, User activity, P.I.I., Financial and payment information & 1 &  \\
%  & Location, User activity, P.I.I., Health information & 1 &  \\
%  & Location, User activity, Web history, P.I.I., Personal communications, Health information & 1 &  \\
%  & Location, Web history, Personal communications & 1 &  \\
%  & Location, Web history, P.I.I., Financial and payment information & 1 &  \\
%  & Location, Website content, Web history, P.I.I., Financial and payment information & 1 &  \\
%  & P.I.I., Financial and payment information, Health information & 1 &  \\
%  & P.I.I., Personal communications, Health information & 1 &  \\
%  & User activity, Web history, P.I.I., Personal communications & 1 &  \\
%  & Web history, P.I.I., Financial and payment information & 1 &  \\
%  & Web history, P.I.I., Personal communications, Health information & 1 &  \\
%  & Website content, Web history, P.I.I., Personal communications, Financial and payment information & 1 &  \\
%  & Website content, Web history, P.I.I., Personal communications, Health information & 1 &  \\ 
% \hline
% \multirow{63}{*}{4} & User activity, Website content & 513 & \multirow{63}{*}{1586} \\
%  & User activity, Website content, P.I.I. & 164 &  \\
%  & User activity, Website content, Web history & 138 &  \\
%  & User activity, Website content, P.I.I., Authentication information & 81 &  \\
%  & Location, User activity, Website content, Web history, P.I.I., Authentication information, Personal communications, Financial and payment information, Health information & 65 &  \\
%  & Location, User activity, Website content & 56 &  \\
%  & Location, User activity, Website content, Web history, P.I.I. & 52 &  \\
%  & Location, User activity, Website content, Web history & 45 &  \\
%  & User activity, Website content, Authentication information & 42 &  \\
%  & User activity, Website content, Web history, P.I.I. & 40 &  \\
%  & Location, User activity, Website content, Web history, Authentication information & 34 &  \\
%  & Location, User activity, Website content, P.I.I., Authentication information, Personal communications & 23 &  \\
%  & Location, User activity, Website content, Web history, P.I.I., Authentication information & 23 &  \\
%  & User activity, Website content, P.I.I., Personal communications & 23 &  \\
%  & Location, User activity, Website content, P.I.I. & 22 &  \\
%  & Location, User activity, Website content, P.I.I., Authentication information & 21 &  \\
%  & Location, User activity, Website content, P.I.I., Personal communications & 20 &  \\
%  & User activity, Website content, Web history, P.I.I., Authentication information & 20 &  \\
%  & Location, User activity, Website content, Web history, P.I.I., Authentication information, Personal communications, Financial and payment information & 19 &  \\
%  & Location, User activity, Website content, Web history, P.I.I., Authentication information, Personal communications & 16 &  \\
%  & User activity, Website content, P.I.I., Authentication information, Financial and payment information & 13 &  \\
%  & Location, User activity, Website content, Web history, P.I.I., Personal communications & 12 &  \\
%  & User activity, Website content, Personal communications & 12 &  \\
%  & User activity, Website content, Web history, Authentication information, Financial and payment information & 12 &  \\
%  & Location, User activity, Website content, Web history, P.I.I., Authentication information, Financial and payment information & 10 &  \\
%  & User activity, Website content, P.I.I., Authentication information, Personal communications & 10 &  \\
%  & User activity, Website content, Web history, Personal communications & 9 &  \\
%  & User activity, Website content, Web history, Authentication information & 8 &  \\
%  & Location, User activity, Website content, P.I.I., Authentication information, Financial and payment information & 6 &  \\
%  & Location, User activity, Website content, P.I.I., Authentication information, Personal communications, Financial and payment information & 5 &  \\
%  & Location, User activity, Website content, Web history, Personal communications & 5 &  \\
%  & User activity, Website content, Web history, P.I.I., Authentication information, Financial and payment information & 5 &  \\
%  & User activity, Website content, Web history, P.I.I., Authentication information, Personal communications & 5 &  \\
%  & Location, User activity, Website content, Personal communications & 4 &  \\
%  & Location, User activity, Website content, Web history, Authentication information, Personal communications & 4 &  \\
%  & User activity, Website content, Web history, P.I.I., Personal communications & 4 &  \\
%  & Location, User activity, Website content, Authentication information & 3 &  \\
%  & Location, User activity, Website content, Web history, P.I.I., Financial and payment information & 3 &  \\
%  & Location, User activity, Website content, Web history, P.I.I., Health information & 3 &  \\
%  & Location, User activity, Website content, Web history, P.I.I., Personal communications, Financial and payment information & 3 &  \\
%  & User activity, Website content, P.I.I., Health information & 3 &  \\
%  & User activity, Website content, Web history, P.I.I., Authentication information, Personal communications, Financial and payment information & 3 &  \\
%  & Location, User activity, Website content, P.I.I., Financial and payment information & 2 &  \\
%  & Location, User activity, Website content, Web history, P.I.I., Authentication information, Health information & 2 &  \\
%  & User activity, Website content, Authentication information, Personal communications & 2 &  \\
%  & User activity, Website content, P.I.I., Authentication information, Personal communications, Financial and payment information & 2 &  \\
%  & User activity, Website content, P.I.I., Financial and payment information & 2 &  \\
%  & User activity, Website content, P.I.I., Personal communications, Financial and payment information & 2 &  \\
%  & Location, User activity, Website content, Financial and payment information & 1 &  \\
%  & Location, User activity, Website content, P.I.I., Health information & 1 &  \\
%  & Location, User activity, Website content, P.I.I., Personal communications, Financial and payment information & 1 &  \\
%  & Location, User activity, Website content, Web history, Personal communications, Financial and payment information, Health information & 1 &  \\
%  & Location, User activity, Website content, Web history, P.I.I., Authentication information, Financial and payment information, Health information & 1 &  \\
%  & Location, User activity, Website content, Web history, P.I.I., Personal communications, Health information & 1 &  \\
%  & User activity, Website content, Authentication information, Financial and payment information & 1 &  \\
%  & User activity, Website content, Financial and payment information & 1 &  \\
%  & User activity, Website content, Health information & 1 &  \\
%  & User activity, Website content, Personal communications, Financial and payment information & 1 &  \\ 
%  & User activity, Website content, P.I.I., Authentication information, Health information & 1 &  \\
%  & User activity, Website content, Web history, Authentication information, Personal communications & 1 &  \\
%  & User activity, Website content, Web history, P.I.I., Authentication information, Health information & 1 &  \\
%  & User activity, Website content, Web history, P.I.I., Authentication information, Personal communications, Health information & 1 &  \\
%  & User activity, Website content, Web history, P.I.I., Personal communications, Health information & 1 &  \\ 
% \hline
% \multirow{18}{*}{5} & User activity & 824 & \multirow{18}{*}{1181} \\
%  & Location, User activity & 118 &  \\
%  & User activity, Web history & 82 &  \\
%  & Location, User activity, Web history & 68 &  \\
%  & User activity, Authentication information & 35 &  \\
%  & User activity, Personal communications & 15 &  \\
%  & Location, User activity, Authentication information, Personal communications & 13 &  \\
%  & Location, User activity, Authentication information & 4 &  \\
%  & Location, User activity, Personal communications & 4 &  \\
%  & User activity, Web history, Authentication information & 4 &  \\
%  & Location, User activity, Web history, Authentication information & 3 &  \\
%  & User activity, Financial and payment information & 3 &  \\
%  & Location, User activity, Web history, Personal communications & 2 &  \\
%  & User activity, Health information & 2 &  \\
%  & Location, User activity, Financial and payment information & 1 &  \\
%  & Location, User activity, Health information & 1 &  \\
%  & User activity, Authentication information, Financial and payment information & 1 &  \\
%  & User activity, Personal communications, Health information & 1 &  \\
% \bottomrule
% \end{tabular}
% }
% \end{table}


\begin{center}
% % \vspace{-2mm}
{\tiny\tabcolsep=3pt
\begin{longtable}{c|lc|l} 
\caption{\bihui{R1.18 Please list the obtained clusters (I'm not sure whether it is clusters for \textbf{all} extensions or \textbf{selected} extensions only)- Obtained clusters }. \heng{I think we don't need to put this table in the paper. We can just use a smaller table to explain each cluster and give an example: four columns (cluster id, explanation and example, total number of extensions, number of extensions sampled. The longer list could be put in the replication package.}}
\label{tab:clusters}\\
% \resizebox{\linewidth}{!}{%

\toprule
\multicolumn{1}{c}{Cluster} & \multicolumn{1}{c}{Privacy Practice} & \multicolumn{1}{c}{Number}  & \multicolumn{1}{c}{Total} \\ \hline
\endfirsthead

\multicolumn{4}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline \multicolumn{1}{c}{Cluster} & \multicolumn{1}{c}{Privacy Practice} & \multicolumn{1}{c}{Number}  & \multicolumn{1}{c}{Total} \\ \hline 
\endhead

\hline \multicolumn{4}{|r|}{{Continued on next page}} \\ \hline
\endfoot

\hline \hline
\endlastfoot

% Cluster & \multicolumn{1}{c}{Privacy Practice} & Number & Total \\ 
% \hline
0 & None & 31908 & 31908 \\ \hline
\multirow{22}{*}{1} & Website content & 3412 & \multirow{22}{*}{4056} \\
 & Website content, Authentication information & 213 &  \\
 & Website content, Web history & 206 &  \\
 & Location, Website content & 88 &  \\
 & Website content, Personal communications & 42 &  \\
 & Location, Website content, Web history & 36 &  \\
 & Location, Website content, Authentication information & 10 &  \\
 & Website content, Authentication information, Personal communications & 10 &  \\
 & Website content, Web history, Authentication information & 10 &  \\
 & Website content, Web history, Personal communications & 6 &  \\
 & Location, Website content, Web history, Authentication information & 4 &  \\
 & Website content, Financial and payment information & 4 &  \\
 & Location, Website content, Financial and payment information & 2 &  \\
 & Location, Website content, Personal communications & 2 &  \\
 & Website content, Authentication information, Financial and payment information & 2 &  \\
 & Website content, Web history, Authentication information, Personal communications & 2 &  \\
 & Website content, Web history, Financial and payment information & 2 &  \\
 & Location, Website content, Authentication information, Personal communications & 1 &  \\
 & Location, Website content, Web history, Personal communications & 1 &  \\
 & Website content, Health information & 1 &  \\
 & Website content, Web history, Authentication information, Health information & 1 &  \\
 & Website content, Web history, Personal communications, Health information & 1 &  \\ 
\hline
\multirow{61}{*}{2} & Authentication information & 492 & \multirow{31}{*}{1951} \\
 & P.I.I. (Personally identifiable information), Authentication information & 432 &  \\
 & Website content, P.I.I., Authentication information & 301 &  \\
 & User activity, P.I.I., Authentication information & 79 &  \\
 & P.I.I., Authentication information, Personal communications & 57 &  \\
 & Location, P.I.I., Authentication information & 54 &  \\
 & P.I.I., Authentication information, Financial and payment information & 54 &  \\
 & Authentication information, Personal communications & 32 &  \\
 & Web history, P.I.I., Authentication information & 31 &  \\
 & Website content, P.I.I., Authentication information, Personal communications & 31 &  \\
 & Location, Authentication information & 26 &  \\
 & Location, Website content, P.I.I., Authentication information & 25 &  \\
 & Location, P.I.I., Authentication information, Financial and payment information & 23 &  \\
 & Location, User activity, P.I.I., Authentication information & 22 &  \\
 & Website content, P.I.I., Authentication information, Financial and payment information & 22 &  \\
 & Website content, Web history, P.I.I., Authentication information & 20 &  \\
 & Location, P.I.I., Authentication information, Personal communications & 17 &  \\
 & User activity, Web history, P.I.I., Authentication information & 17 &  \\
 & Location, User activity, P.I.I., Authentication information, Financial and payment information & 16 &  \\
 & P.I.I., Authentication information, Personal communications, Financial and payment information & 16 &  \\
 & User activity, P.I.I., Authentication information, Financial and payment information & 16 &  \\
 & Location, Website content, Web history, P.I.I., Authentication information & 15 &  \\
 & Web history, Authentication information & 15 &  \\
 & Authentication information, Financial and payment information & 13 &  \\
 & User activity, P.I.I., Authentication information, Personal communications & 12 &  \\
 & Website content, Web history, P.I.I., Authentication information, Personal communications & 10 &  \\
 & Location, Website content, P.I.I., Authentication information, Personal communications & 7 &  \\
 & Website content, P.I.I., Authentication information, Personal communications, Financial and payment information & 7 &  \\
 & Location, User activity, P.I.I., Authentication information, Personal communications, Financial and payment information & 6 &  \\
 & Location, User activity, Web history, P.I.I., Authentication information & 6 &  \\
 & Location, Web history, P.I.I., Authentication information & 6 &  \\
 & Location, P.I.I., Authentication information, Personal communications, Financial and payment information & 5 &  \\
 & Web history, P.I.I., Authentication information, Financial and payment information & 5 &  \\
 & Website content, Web history, P.I.I., Authentication information, Financial and payment information & 5 &  \\
 & Authentication information, Personal communications, Financial and payment information & 4 &  \\
 & Location, User activity, P.I.I., Authentication information, Personal communications & 4 &  \\
 & Location, Web history, Authentication information & 4 &  \\
 & Location, Web history, P.I.I., Authentication information, Financial and payment information & 4 &  \\
 & Location, Website content, P.I.I., Authentication information, Financial and payment information & 4 &  \\
 & Location, P.I.I., Authentication information, Financial and payment information, Health information & 3 &  \\
 & Location, User activity, Web history, P.I.I., Authentication information, Personal communications, Financial and payment information & 3 &  \\
 & Location, Web history, P.I.I., Authentication information, Personal communications & 3 &  \\
 & Location, Authentication information, Personal communications & 2 &  \\
 & Location, User activity, Web history, P.I.I., Authentication information, Financial and payment information & 2 &  \\
 & Location, Website content, P.I.I., Authentication information, Personal communications, Financial and payment information & 2 &  \\
 & P.I.I., Authentication information, Health information & 2 &  \\
 & P.I.I., Authentication information, Personal communications, Health information & 2 &  \\
 & Web history, Authentication information, Personal communications & 2 &  \\
 & Web history, P.I.I., Authentication information, Personal communications & 2 &  \\
 & Website content, Web history, P.I.I., Authentication information, Personal communications, Financial and payment information & 2 &  \\
 & Location, Authentication information, Financial and payment information & 1 &  \\
 & Location, P.I.I., Authentication information, Health information & 1 &  \\
 & Location, P.I.I., Authentication information, Personal communications, Health information & 1 &  \\
 & Location, User activity, Web history, P.I.I., Authentication information, Personal communications & 1 &  \\
 & Location, Website content, Web history, P.I.I., Authentication information, Personal communications & 1 &  \\
 & Location, Website content, Web history, P.I.I., Authentication information, Personal communications, Financial and payment information, Health information & 1 &  \\
 & P.I.I., Authentication information, Personal communications, Financial and payment information, Health information & 1 &  \\
 & User activity, P.I.I., Authentication information, Health information & 1 &  \\
 & User activity, P.I.I., Authentication information, Personal communications, Financial and payment information & 1 &  \\
 & User activity, Web history, P.I.I., Authentication information, Personal communications & 1 &  \\
 & Website content, P.I.I., Authentication information, Health information & 1 &  \\ 
\hline
\multirow{59}{*}{3} & P.I.I. & 1490 & \multirow{59}{*}{3649} \\
 & Website content, P.I.I. & 449 &  \\
 & Web history & 368 &  \\
 & Location & 338 &  \\
 & User activity, P.I.I. & 121 &  \\
 & Personal communications & 116 &  \\
 & P.I.I., Personal communications & 107 &  \\
 & Location, P.I.I. & 85 &  \\
 & Web history, P.I.I. & 83 &  \\
 & Location, Web history & 53 &  \\
 & Website content, P.I.I., Personal communications & 52 &  \\
 & Website content, Web history, P.I.I. & 46 &  \\
 & Location, Website content, P.I.I. & 36 &  \\
 & P.I.I., Financial and payment information & 34 &  \\
 & Location, User activity, P.I.I. & 31 &  \\
 & Location, Web history, P.I.I. & 23 &  \\
 & Financial and payment information & 21 &  \\
 & User activity, Web history, P.I.I. & 20 &  \\
 & Location, Website content, Web history, P.I.I. & 15 &  \\
 & Website content, P.I.I., Financial and payment information & 15 &  \\
 & Location, Personal communications & 12 &  \\
 & Location, P.I.I., Personal communications & 12 &  \\
 & Location, User activity, Web history, P.I.I. & 12 &  \\
 & Location, Website content, P.I.I., Personal communications & 12 &  \\
 & User activity, P.I.I., Personal communications & 11 &  \\
 & Health information & 8 &  \\
 & Location, User activity, P.I.I., Personal communications & 8 &  \\
 & User activity, P.I.I., Financial and payment information & 7 &  \\
 & P.I.I., Personal communications, Financial and payment information & 6 &  \\
 & Location, P.I.I., Financial and payment information & 5 &  \\
 & P.I.I., Health information & 4 &  \\
 & Website content, Web history, P.I.I., Personal communications & 4 &  \\
 & Location, User activity, P.I.I., Personal communications, Financial and payment information & 3 &  \\
 & Location, User activity, Web history, P.I.I., Personal communications & 3 &  \\
 & Location, Web history, P.I.I., Personal communications & 3 &  \\
 & Web history, Personal communications & 3 &  \\
 & Location, P.I.I., Personal communications, Financial and payment information & 2 &  \\
 & Location, User activity, Web history, P.I.I., Financial and payment information & 2 &  \\
 & Location, Website content, P.I.I., Financial and payment information & 2 &  \\
 & Location, Website content, P.I.I., Personal communications, Financial and payment information & 2 &  \\
 & Location, Website content, Web history, P.I.I., Personal communications & 2 &  \\
 & User activity, P.I.I., Personal communications, Financial and payment information & 2 &  \\
 & Web history, P.I.I., Personal communications & 2 &  \\
 & Website content, P.I.I., Health information & 2 &  \\
 & Website content, P.I.I., Personal communications, Financial and payment information & 2 &  \\
 & Website content, Web history, P.I.I., Financial and payment information & 2 &  \\
 & Location, User activity, P.I.I., Financial and payment information & 1 &  \\
 & Location, User activity, P.I.I., Health information & 1 &  \\
 & Location, User activity, Web history, P.I.I., Personal communications, Health information & 1 &  \\
 & Location, Web history, Personal communications & 1 &  \\
 & Location, Web history, P.I.I., Financial and payment information & 1 &  \\
 & Location, Website content, Web history, P.I.I., Financial and payment information & 1 &  \\
 & P.I.I., Financial and payment information, Health information & 1 &  \\
 & P.I.I., Personal communications, Health information & 1 &  \\
 & User activity, Web history, P.I.I., Personal communications & 1 &  \\
 & Web history, P.I.I., Financial and payment information & 1 &  \\
 & Web history, P.I.I., Personal communications, Health information & 1 &  \\
 & Website content, Web history, P.I.I., Personal communications, Financial and payment information & 1 &  \\
 & Website content, Web history, P.I.I., Personal communications, Health information & 1 &  \\ 
\hline
\multirow{63}{*}{4} & User activity, Website content & 513 & \multirow{63}{*}{1586} \\
 & User activity, Website content, P.I.I. & 164 &  \\
 & User activity, Website content, Web history & 138 &  \\
 & User activity, Website content, P.I.I., Authentication information & 81 &  \\
 & Location, User activity, Website content, Web history, P.I.I., Authentication information, Personal communications, Financial and payment information, Health information & 65 &  \\
 & Location, User activity, Website content & 56 &  \\
 & Location, User activity, Website content, Web history, P.I.I. & 52 &  \\
 & Location, User activity, Website content, Web history & 45 &  \\
 & User activity, Website content, Authentication information & 42 &  \\
 & User activity, Website content, Web history, P.I.I. & 40 &  \\
 & Location, User activity, Website content, Web history, Authentication information & 34 &  \\
 & Location, User activity, Website content, P.I.I., Authentication information, Personal communications & 23 &  \\
 & Location, User activity, Website content, Web history, P.I.I., Authentication information & 23 &  \\
 & User activity, Website content, P.I.I., Personal communications & 23 &  \\
 & Location, User activity, Website content, P.I.I. & 22 &  \\
 & Location, User activity, Website content, P.I.I., Authentication information & 21 &  \\
 & Location, User activity, Website content, P.I.I., Personal communications & 20 &  \\
 & User activity, Website content, Web history, P.I.I., Authentication information & 20 &  \\
 & Location, User activity, Website content, Web history, P.I.I., Authentication information, Personal communications, Financial and payment information & 19 &  \\
 & Location, User activity, Website content, Web history, P.I.I., Authentication information, Personal communications & 16 &  \\
 & User activity, Website content, P.I.I., Authentication information, Financial and payment information & 13 &  \\
 & Location, User activity, Website content, Web history, P.I.I., Personal communications & 12 &  \\
 & User activity, Website content, Personal communications & 12 &  \\
 & User activity, Website content, Web history, Authentication information, Financial and payment information & 12 &  \\
 & Location, User activity, Website content, Web history, P.I.I., Authentication information, Financial and payment information & 10 &  \\
 & User activity, Website content, P.I.I., Authentication information, Personal communications & 10 &  \\
 & User activity, Website content, Web history, Personal communications & 9 &  \\
 & User activity, Website content, Web history, Authentication information & 8 &  \\
 & Location, User activity, Website content, P.I.I., Authentication information, Financial and payment information & 6 &  \\
 & Location, User activity, Website content, P.I.I., Authentication information, Personal communications, Financial and payment information & 5 &  \\
 & Location, User activity, Website content, Web history, Personal communications & 5 &  \\
 & User activity, Website content, Web history, P.I.I., Authentication information, Financial and payment information & 5 &  \\
 & User activity, Website content, Web history, P.I.I., Authentication information, Personal communications & 5 &  \\
 & Location, User activity, Website content, Personal communications & 4 &  \\
 & Location, User activity, Website content, Web history, Authentication information, Personal communications & 4 &  \\
 & User activity, Website content, Web history, P.I.I., Personal communications & 4 &  \\
 & Location, User activity, Website content, Authentication information & 3 &  \\
 & Location, User activity, Website content, Web history, P.I.I., Financial and payment information & 3 &  \\
 & Location, User activity, Website content, Web history, P.I.I., Health information & 3 &  \\
 & Location, User activity, Website content, Web history, P.I.I., Personal communications, Financial and payment information & 3 &  \\
 & User activity, Website content, P.I.I., Health information & 3 &  \\
 & User activity, Website content, Web history, P.I.I., Authentication information, Personal communications, Financial and payment information & 3 &  \\
 & Location, User activity, Website content, P.I.I., Financial and payment information & 2 &  \\
 & Location, User activity, Website content, Web history, P.I.I., Authentication information, Health information & 2 &  \\
 & User activity, Website content, Authentication information, Personal communications & 2 &  \\
 & User activity, Website content, P.I.I., Authentication information, Personal communications, Financial and payment information & 2 &  \\
 & User activity, Website content, P.I.I., Financial and payment information & 2 &  \\
 & User activity, Website content, P.I.I., Personal communications, Financial and payment information & 2 &  \\
 & Location, User activity, Website content, Financial and payment information & 1 &  \\
 & Location, User activity, Website content, P.I.I., Health information & 1 &  \\
 & Location, User activity, Website content, P.I.I., Personal communications, Financial and payment information & 1 &  \\
 & Location, User activity, Website content, Web history, Personal communications, Financial and payment information, Health information & 1 &  \\
 & Location, User activity, Website content, Web history, P.I.I., Authentication information, Financial and payment information, Health information & 1 &  \\
 & Location, User activity, Website content, Web history, P.I.I., Personal communications, Health information & 1 &  \\
 & User activity, Website content, Authentication information, Financial and payment information & 1 &  \\
 & User activity, Website content, Financial and payment information & 1 &  \\
 & User activity, Website content, Health information & 1 &  \\
 & User activity, Website content, Personal communications, Financial and payment information & 1 &  \\ 
% \cline{2-2}
 & User activity, Website content, P.I.I., Authentication information, Health information & 1 &  \\
 & User activity, Website content, Web history, Authentication information, Personal communications & 1 &  \\
 & User activity, Website content, Web history, P.I.I., Authentication information, Health information & 1 &  \\
 & User activity, Website content, Web history, P.I.I., Authentication information, Personal communications, Health information & 1 &  \\
 & User activity, Website content, Web history, P.I.I., Personal communications, Health information & 1 &  \\ 
\hline
\multirow{18}{*}{5} & User activity & 824 & \multirow{18}{*}{1181} \\
 & Location, User activity & 118 &  \\
 & User activity, Web history & 82 &  \\
 & Location, User activity, Web history & 68 &  \\
 & User activity, Authentication information & 35 &  \\
 & User activity, Personal communications & 15 &  \\
 & Location, User activity, Authentication information, Personal communications & 13 &  \\
 & Location, User activity, Authentication information & 4 &  \\
 & Location, User activity, Personal communications & 4 &  \\
 & User activity, Web history, Authentication information & 4 &  \\
 & Location, User activity, Web history, Authentication information & 3 &  \\
 & User activity, Financial and payment information & 3 &  \\
 & Location, User activity, Web history, Personal communications & 2 &  \\
 & User activity, Health information & 2 &  \\
 & Location, User activity, Financial and payment information & 1 &  \\
 & Location, User activity, Health information & 1 &  \\
 & User activity, Authentication information, Financial and payment information & 1 &  \\
 & User activity, Personal communications, Health information & 1 &  \\
\bottomrule
\end{longtable}
}
% % }
\end{center}

==> tables/rq2.tex <==
\begin{table}
\vspace{-2mm}
\centering
%\caption{Statistical performance changes of the extensions in different activation modes of extensions}
\caption{Comparing the performance impact of different activation modes of the extensions with the extension-free mode and the fully-loaded mode.} 
% \heng{missing some data in the table: if the count is zero, put 0 for count and - for ratio} 
% \heng{double check the comparison results between fully inactive and fully loaded modes, for page load energy consumption and stabilized energy consumption (numbers in brackets for ``increase'' are bigger, looking suspicious); also the comparisons between non-designated and fully loaded, for the stabilized energy consumption.}}

\vspace{-2mm}
\label{tab:mode-result2}\label{tab:mode-result}
\resizebox{\linewidth}{!}{
% \begin{tabular}{l|c|cr|cr|cr|cr|cr} 
% \hline
% \multicolumn{2}{c|}{Mode}                                                                            & \multicolumn{2}{c|}{Fully Loaded}  & \multicolumn{2}{c|}{No Grant}                          & \multicolumn{2}{c|}{No Login}                          & \multicolumn{2}{c|}{Inactive}                          & \multicolumn{2}{c}{Fully Inactive}                     \\ 
% \hline
% \begin{tabular}[c]{@{}l@{}}Performance\\metrics\end{tabular}                              & Tendency & Count & \multicolumn{1}{c|}{Ratio} & \multicolumn{1}{l}{Count} & \multicolumn{1}{c|}{Ratio} & \multicolumn{1}{l}{Count} & \multicolumn{1}{c|}{Ratio} & \multicolumn{1}{l}{Count} & \multicolumn{1}{c|}{Ratio} & \multicolumn{1}{l}{Count} & \multicolumn{1}{c}{Ratio}  \\ 
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Page load\\time\end{tabular}}                  & Increase & 16    & 18.07\%                    & 1                         & 13.37\%                    & 1                         & 33.16\%                    & 1                         & 335.48\%                   & 4                         & 231.28\%                   \\ 
% \cline{2-2}
%                                                                                           & Decrease & 16    & -7.16\%                    & 4                         & -6.92\%                    & 1                         & -7.08\%                    &                           &                            & 3                         & -36.26\%                   \\ 
% \cline{2-2}
%                                                                                           & Overall  & 32    & 1.00\%                     & 5                         & -6.51\%                    & 2                         & 13.04\%                    & 1                         & 335.48\%                   & 7                         & 80.27\%                    \\ 
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Page load\\energy\\consumption\end{tabular}}   & Increase & 36    & 17.12\%                    & 4                         & 14.82\%                    & 7                         & 11.53\%                    & 5                         & 14.46\%                    & 4                         & 577.49\%                   \\ 
% \cline{2-2}
%                                                                                           & Decrease & 4     & -6.61\%                    &                           &                            &                           &                            &                           &                            & 3                         & -28.89\%                   \\ 
% \cline{2-2}
%                                                                                           & Overall  & 40    & 15.57\%                    & 4                         & 14.82\%                    & 7                         & 11.53\%                    & 5                         & 14.46\%                    & 7                         & 11.69\%                    \\ 
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Stabilized \\energy\\consumption\end{tabular}} & Increase & 38    & 1.73\%                     & 9                         & 2.81\%                     & 8                         & 2.72\%                     & 3                         & 1.56\%                     & 8                         & 13.04\%                    \\ 
% \cline{2-2}
%                                                                                           & Decrease & 6     & -1.58\%                    &                           &                            &                           &                            & 5                         & -0.79\%                    & 3                         & -27.75\%                   \\ 
% \cline{2-2}
%                                                                                           & Overall  & 44    & 1.44\%                     & 9                         & 2.81\%                     & 8                         & 2.72\%                     & 8                         & -0.47\%                    & 11                        & 8.79\%                     \\ 
% \hline
% \multicolumn{2}{l|}{\# of extensions being tested}                                                   & \multicolumn{2}{c|}{61}            & \multicolumn{2}{c|}{10}                                & \multicolumn{2}{c|}{8}                                 & \multicolumn{2}{c|}{11}                                & \multicolumn{2}{c}{11}                                 \\
% \hline
% \end{tabular}
\begin{threeparttable}
\begin{tabular}{l|c|cr|cr|cr|cr} 
\hline
\multicolumn{2}{c|}{Mode}                                                                            & \multicolumn{2}{c|}{No-grant}                                                                                & \multicolumn{2}{c|}{No-login}                                                                                 & \multicolumn{2}{c|}{Non-designated}                                                                         & \multicolumn{2}{c}{Fully-inactive}                                                                               \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Performance\\ metrics\end{tabular}                             & Tendency & \multicolumn{1}{l}{Count}                       & \multicolumn{1}{c|}{Ratio}                                 & \multicolumn{1}{l}{Count}                        & \multicolumn{1}{c|}{Ratio}                                 & \multicolumn{1}{l}{Count}                      & \multicolumn{1}{c|}{Ratio}                                 & \multicolumn{1}{l}{Count}                        & \multicolumn{1}{c}{Ratio}                                     \\ 
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Page load\\time\end{tabular}}                  & Increase & \begin{tabular}[c]{@{}c@{}}2\\(1)\end{tabular}  & \begin{tabular}[c]{@{}r@{}}43.16\%\\(17.31\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}5\\(3)\end{tabular}   & \begin{tabular}[c]{@{}r@{}}46.34\%\\(17.30\%)\end{tabular} & 1                                              & 335.48\%                                                   & \begin{tabular}[c]{@{}c@{}}4\\(4)\end{tabular}   & \begin{tabular}[c]{@{}r@{}}231.28\%\\(21.25\%)\end{tabular}   \\ 
\cline{2-2}
                                                                                          & Decrease & \begin{tabular}[c]{@{}c@{}}4\\(3)\end{tabular}  & \begin{tabular}[c]{@{}r@{}}-6.92\%\\(-3.07\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}2\\(2)\end{tabular}   & \begin{tabular}[c]{@{}r@{}}-4.83\%\\(-7.39\%)\end{tabular} & 0                                              & \multicolumn{1}{c|}{-}                                     & \begin{tabular}[c]{@{}c@{}}3\\(2)\end{tabular}   & \begin{tabular}[c]{@{}r@{}}-36.26\%\\(-40.87\%)\end{tabular}  \\ 
\cline{2-2}
                                                                                          & Overall  & \begin{tabular}[c]{@{}c@{}}6\\(4)\end{tabular}  & \begin{tabular}[c]{@{}r@{}}-6.35\%\\(-2.06\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}7\\(5)\end{tabular}   & \begin{tabular}[c]{@{}r@{}}33.16\%\\(7.02\%)\end{tabular}  & 1                                              & 335.48\%                                                   & \begin{tabular}[c]{@{}c@{}}7\\(6)\end{tabular}   & \begin{tabular}[c]{@{}r@{}}80.27\%\\(11.06\%)\end{tabular}    \\ 
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Page load\\energy\\consumption\end{tabular}}   & Increase & \begin{tabular}[c]{@{}c@{}}5\\(1)\end{tabular}  & \begin{tabular}[c]{@{}r@{}}18.95\%\\(44.41\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}12\\(9)\end{tabular}  & \begin{tabular}[c]{@{}r@{}}18.45\%\\(18.51\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}5\\(3)\end{tabular} & \begin{tabular}[c]{@{}r@{}}14.46\%\\(10.68\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}4\\(6)\end{tabular}   & \begin{tabular}[c]{@{}r@{}}577.49\%\\(13.54\%)\end{tabular}   \\ 
\cline{2-2}
                                                                                          & Decrease & 0                                               & \multicolumn{1}{c|}{-}                                     & 0                                                & \multicolumn{1}{c|}{-}                                     & \begin{tabular}[c]{@{}c@{}}\\(1)\end{tabular}  & \begin{tabular}[c]{@{}r@{}}\\(-60.92\%)\end{tabular}       & \begin{tabular}[c]{@{}c@{}}3\\(1)\end{tabular}   & \begin{tabular}[c]{@{}r@{}}-28.89\%\\(-5.88\%)\end{tabular}   \\ 
\cline{2-2}
                                                                                          & Overall  & \begin{tabular}[c]{@{}c@{}}5\\(1)\end{tabular}  & \begin{tabular}[c]{@{}r@{}}18.95\%\\(44.41\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}12\\(9)\end{tabular}  & \begin{tabular}[c]{@{}r@{}}18.45\%\\(18.51\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}5\\(4)\end{tabular} & \begin{tabular}[c]{@{}r@{}}14.46\%\\(7.95\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}7\\(7)\end{tabular}   & \begin{tabular}[c]{@{}r@{}}11.69\%\\(10.68\%)\end{tabular}    \\ 
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Stabilized \\energy\\consumption\end{tabular}} & Increase & \begin{tabular}[c]{@{}c@{}}11\\(7)\end{tabular} & \begin{tabular}[c]{@{}r@{}}2.81\%\\(3.99\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}15\\(9)\end{tabular}  & \begin{tabular}[c]{@{}r@{}}2.93\%\\(1.63\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}3\\(7)\end{tabular} & \begin{tabular}[c]{@{}r@{}}1.56\%\\(1.33\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}8\\(9)\end{tabular}   & \begin{tabular}[c]{@{}r@{}}13.04\%\\(1.35\%)\end{tabular}     \\ 
\cline{2-2}
                                                                                          & Decrease & 0                                               & \multicolumn{1}{c|}{-}                                     & \begin{tabular}[c]{@{}c@{}}\\(1)\end{tabular}    & \begin{tabular}[c]{@{}r@{}}\\(-0.83\%)\end{tabular}        & 5                                              & -0.79\%                                                    & \begin{tabular}[c]{@{}c@{}}3\\(1)\end{tabular}   & \begin{tabular}[c]{@{}r@{}}-27.75\%\\(-3.84\%)\end{tabular}   \\ 
\cline{2-2}
                                                                                          & Overall  & \begin{tabular}[c]{@{}c@{}}11\\(7)\end{tabular} & \begin{tabular}[c]{@{}r@{}}2.81\%\\(3.99\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}15\\(10)\end{tabular} & \begin{tabular}[c]{@{}r@{}}2.93\%\\(1.58\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}8\\(7)\end{tabular} & \begin{tabular}[c]{@{}r@{}}-0.47\%\\(1.33\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}11\\(10)\end{tabular} & \begin{tabular}[c]{@{}r@{}}8.79\%\\(1.34\%)\end{tabular}      \\ 
\hline
\multicolumn{2}{l|}{\# of extensions being tested}                                                   & \multicolumn{2}{c|}{13}                                                                                      & \multicolumn{2}{c|}{17}                                                                                       & \multicolumn{2}{c|}{11}                                                                                     & \multicolumn{2}{c}{11}                                                                                           \\
\hline
\end{tabular}
\begin{tablenotes}
      \normalsize
      \item The figures outside and inside the brackets indicate the results of comparing the activation modes with the extension-free mode and the fully-loaded mode, respectively. % The bracketed figures indicate the change ratio of corresponding extensions in each activation mode found in the fully loaded mode.
      \item Due to space limitation, we share our Cliff's delta results in our replication package.
      % \heng{Only mention this as a table note in Table 4} 
\end{tablenotes}
\end{threeparttable}
% \begin{tabular}{l|l|lrlrlrlr|lrlrlrlr} 
% \hline
% \multicolumn{2}{l|}{Mode}                                                                                   & \multicolumn{8}{c|}{Inactive}                                                                                                                                                                          & \multicolumn{8}{c}{Fully Inactive}                                                                                                                                                                     \\ 
% \hline
% \multicolumn{2}{l|}{Cliff’s $\delta$}                                                                              & \multicolumn{2}{c}{Diff}                        & \multicolumn{2}{c}{Small}                       & \multicolumn{2}{c}{Medium}                      & \multicolumn{2}{c|}{Large}                       & \multicolumn{2}{c}{Diff}                        & \multicolumn{2}{c}{Small}                       & \multicolumn{2}{c}{Medium}                      & \multicolumn{2}{c}{Large}                        \\ 
% \hline
% Attribute                                                                                      & Change ratio & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{\%} & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{\%} & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{\%} & \multicolumn{1}{c}{\#} & \multicolumn{1}{c|}{\%} & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{\%} & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{\%} & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{\%} & \multicolumn{1}{c}{\#} & \multicolumn{1}{c}{\%}  \\ 
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Response \\ time of \\ payload\end{tabular}}     & Increase     & 1                      & 335.48\%               &                        & \multicolumn{1}{l}{}   &                        & \multicolumn{1}{l}{}   & 1                      & 335.48\%                & 4                      & 231.28\%               & 2                      & 109.07\%               & 1                      & 324.68\%               & 1                      & 716.16\%                \\ 
% \cline{2-2}
%                                                                                              & Decrease         &                        &                        &                        & \multicolumn{1}{l}{}   &                        & \multicolumn{1}{l}{}   &                        &                         & 3                      & -36.26\%               &                        &                        & 2                      & -34.07\%               & 1                      & -60.11\%                \\ 
% \cline{2-2}
%                                                                                              & Overall      & 1                      & 335.48\%               &                        & \multicolumn{1}{l}{}   &                        & \multicolumn{1}{l}{}   & 1                      & 335.48\%                & 7                      & 80.27\%                & 2                      & 109.07\%               & 3                      & -31.89\%               & 2                      & 328.02\%                \\ 
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Energy \\ consumption \\ of payload\end{tabular}}    & Increase     & 5                      & 14.46\%                & 3                      & 10.19\%                & 1                      & 14.98\%                & 1                      & 728.47\%                & 4                      & 577.49\%               & 1                      & 11.69\%                & 1                      & 283.53\%               & 2                      & 1376.72\%               \\ 
% \cline{2-2}
%                                                                                              & Decrease         &                        &                        &                        &                        &                        &                        &                        &                         & 3                      & -28.89\%               & 1                      & -4.10\%                & 2                      & -38.41\%               &                        &                         \\ 
% \cline{2-2}
%                                                                                              & Overall      & 5                      & 14.46\%                & 3                      & 10.19\%                & 1                      & 14.98\%                & 1                      & 728.47\%                & 7                      & 11.69\%                & 2                      & 3.80\%                 & 3                      & -28.89\%               & 2                      & 1376.72\%               \\ 
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Stabilized \\ energy \\ consumption\end{tabular}} & Increase     & 3                      & 1.56\%                 &                        &                        & 2                      & 1.06\%                 & 1                      & 43.16\%                 & 8                      & 13.04\%                & 2                      & 6.66\%                 & 3                      & 14.18\%                & 3                      & 19.28\%                 \\ 
% \cline{2-2}
%                                                                                              & Decrease         & 5                      & -0.79\%                & 5                      & -0.79\%                &                        &                        &                        &                         & 3                      & -27.75\%               &                        &                        &                        &                        & 3                      & -27.75\%                \\ 
% \cline{2-2}
%                                                                                              & Overall      & 8                      & -0.47\%                & 5                      & -0.79\%                & 2                      & 1.06\%                 & 1                      & 43.16\%                 & 11                     & 8.79\%                 & 2                      & 6.66\%                 & 3                      & 14.18\%                & 6                      & -7.23\%                 \\ 
% \hline
% \multicolumn{2}{l|}{\# of extensions being tested}                                                          & \multicolumn{8}{c|}{11}                                                                                                                                                                                & \multicolumn{8}{c}{11}                                                                                                                                                                                 \\
% \hline
% \end{tabular}
}
\vspace{-8mm}
\end{table}

==> texts/06_implication.tex <==
In this section, we discuss the implications of our findings for extension users, extension developers, and future researchers.

\subsection{Implication for Extension Users}
\textbf{Extension users should be aware of the performance ramifications associated with different activation modes of extensions to optimize their configurations of the extensions.}
\bihui{As noted in the findings of RQ1 (Section \ref{rq1}) and RQ2 (Section \ref{rq2}), browser performance is negatively impacted by the use of extensions, irrespective of the specific activation mode of extensions. 
Such an observation implies that even when extensions are not activated, they can still adversely impact the browser performance.
\bj{Findings from RQ2 could contribute to establishing best practices for extension users.}
Extension users should carefully consider the activation mode of extensions while using the extension and only activate the extension that is indispensable. 
Moreover, they should also periodically scrutinize their extensions and remove any that are no longer needed.
By optimizing the configurations of the using extensions, users can improve the overall performance and refine the user browsing experience by reducing page load time and minimizing energy consumption.}

% \bihui{Findings from this RQ could contribute to establishing best practices for extension development. 
% Developers can gain insights into which activation modes are more likely to influence performance and consider these factors during the development process, leading to more efficient and reliable extensions.
% Additionally, users can become more aware of the potential additional energy expenses associated with different activation modes, ultimately improving their browsing experience and minimizing energy consumption.}
\textbf{Extension users could select fungible extensions that have minimal impact on browser performance.} 
\bihui{As highlighted in the findings of RQ3 (Section \ref{rq3}), we discuss the factors that have a correlation with performance changes.
Extension users can select a substitute that offers similar functionality with less impact on the browser performance based on the affecting trend of these factors (e.g., privacy practices or extension size) that we find in RQ3.
By selecting extensions that have less performance-impacted factors, users can mitigate the negative impact on browser performance while still enjoying the functionality they need.}

\subsection{Implication for Browser and Extension Developers}
\textbf{Browser and extension developers should pay attention to the performance impact of browser extensions, particularly in regard to energy efficiency.} 
\bihui{In RQ2 (Section \ref{rq2}), we find that using extensions can cause performance deterioration to the browser, which may lead to a poor user experience. 
Therefore, it is crucial that browser and extension developers prioritize optimizing the performance of their extensions to ensure that their extensions consume minimal resources while still providing the intended functionalities to the users. 
\bj{In addition, developers can gain insights into which activation modes are more likely to influence performance and consider these factors during the development process, leading to more efficient and reliable extensions.}
To enhance user satisfaction and decrease the negative impact on the browser performance, we recommend browser and extension developers to take heed of the performance impact of browser extensions by improving the code quality, prioritizing essential content, optimizing resource loading, minimizing data transfers, and utilizing proper privacy practices for the extension. 
Furthermore, they should regularly maintain their extensions to ensure that extensions are up-to-date and compatible with the latest browser versions. }

\subsection{Implication for Future Research}
\textbf{Researchers, who focused on performance and energy profiling, could provide mechanisms to mitigate the adverse performance impact of extensions that fail to provide proper functionalities (e.g., when in a non-designated mode) to users, particularly when they are in a fully inactive mode.} 
\bihui{As discussed in RQ3 (Section \ref{rq3}), popular extensions (i.e., more users to download) tend to consume more energy, while extensions with a larger extension size tend to lower energy consumption. 
Privacy practices used within extensions can also have varying impacts on the browser performance.
Future researchers could verify that whether poorly optimized extensions can consume significant amounts of energy and slow down the browser. 
Such effects can be particularly troublesome for users who have multiple extensions installed, as the cumulative effect of extensions can lead to significant performance degradation. 
Hence, it is recommended that performance and energy profiling researchers could use our proposed approach in RQ3 to develop mechanisms that can detect when an extension is not being used or not providing useful functionalities to users and automatically deactivate such extension to reduce the performance impact of extensions.} 
\bj{Moreover, future work may extend our work by evaluating the performance impact of extensions on other browsers.}

